Grasping Field: Learning Implicit Representations for Human Grasps

Robotic grasping of house-hold objects has made remarkable progress in recent years. Yet, human grasps are still difficult to synthesize realistically. There are several key reasons: (1) the human hand has many degrees of freedom (more than robotic manipulators); (2) the synthesized hand should conform to the surface of the object; and (3) it should interact with the object in a semantically and physically plausible manner. To make progress in this direction, we draw inspiration from the recent progress on learning-based implicit representations for 3D object reconstruction. Specifically, we propose an expressive representation for human grasp modelling that is efficient and easy to integrate with deep neural networks. Our insight is that every point in a three-dimensional space can be characterized by the signed distances to the surface of the hand and the object, respectively. Consequently, the hand, the object, and the contact area can be represented by implicit surfaces in a common space, in which the proximity between the hand and the object can be modelled explicitly. We name this 3D to 2D mapping as Grasping Field, parameterize it with a deep neural network, and learn it from data. We demonstrate that the proposed grasping field is an effective and expressive representation for human grasp generation. Specifically, our generative model is able to synthesize high-quality human grasps, given only on a 3D object point cloud. The extensive experiments demonstrate that our generative model compares favorably with a strong baseline and approaches the level of natural human grasps. Our method improves the physical plausibility of the hand-object contact reconstruction and achieves comparable performance for 3D hand reconstruction compared to state-of-the-art methods.

==> Grasping Field - 3DV/Sec1-Introduction.tex <==
\section{Introduction}
\label{sec:intro}

%Humans manipulate the world mostly with their hands. 
%\begin{figure}
%    \centering
%    \includegraphics[width=0.8\linewidth]{Figure/teaser.png}
%    \caption{From left to right in each row: The RGB image \cite{zimmermann2019freihand}, the hand-object reconstruction, and 5 generated hand grasps based on the same object. Note that our reconstruction model is only trained on the ObMan dataset \cite{hasson2019obman}.}
%    \label{fig:teaser}
%\end{figure}

%Humans interact with real-world objects using hands, and such interaction is rooted in the physical hand-object contact.
%Through this contact, humans are able to grasp and manipulate objects naturally.

Capturing and synthesizing hand-object interaction is essential for understanding human behaviours, and is key to a number of applications including augmented and virtual reality, robotics and human-computer interaction.  
% Despite a tremendous progress in the past, reconstructing hand from an RGB image while simultaneously taking into account the object that is in contact with it remains an extremely challenging problem. 
%Despite tremendous progress, reconstructing the hands from an RGB image together with an object it is holding and the contact between them remains an extremely challenging problem. 
Despite substantial progress, fully automatic synthesis of highly realistic human grasps remains an unsolved problem. The anatomical complexity of the human hand and the variety of manufactured and natural objects make it extremely challenging to pose the hand such that it interacts with the object in a natural and physically plausible way. Recent data-driven approaches explore deep learning technology to learn and leverage powerful object representations, yet they are mainly limited to simple robotic end effectors, such as parallel jaw grippers \cite{7139361}. In this work, we seek to understand: 1) what is an efficient and expressive representation for modeling hand-object interaction, that can facilitate realistic human grasp synthesis given an unseen 3D object; and 2) how can we learn such a representation from data. 



Our key observation is that human grasping is rooted in physical hand-object {\em contact}. Through this contact, humans are able to grasp and manipulate objects naturally. To better model hand-object interaction, we must find a way to effectively represent the contact between hands and objects. 
To this end, we propose a novel interaction representation that is based on regressing a continuous function that we call the {\it Grasping Field}. The grasping field maps any 3D point to a 2D space, where each dimension of the 2D space indicates the signed distance to the surface of the hand and the object respectively (see Sec.~\ref{sec:gf_definition} for a formal definition).
Inspired by \cite{mescheder2019occupancy,OechsleICCV2019,park2019deepsdf}, we further utilize a deep neural network to parameterize the grasping field and learn it from data. 
As a result, the learned grasping field serves as a powerful representation to facilitate hand-object interaction modelling. 


% generative model
Based on the grasping field representation, we propose a generative model, in which we generate plausible hand grasps given an object point cloud.  
We show that our model can produce physically and semantically plausible synthetic grasps, which are similar to the ground truth. Generated grasps on unseen objects are shown in Fig.~\ref{fig:generative} and Fig.~\ref{fig:sample_ho3d}.

%reconstruction model
We further demonstrate the effectiveness of the grasping field representation by considering the task of 3D hand and object reconstruction from a single RGB image.
In recent work, Hasson et al.~\cite{hasson2019obman} introduce an end-to-end learnable model to reconstruct 3D meshes of the hand and object simultaneously, producing the state-of-the-art results on several datasets. Physical constraints, such as no interpenetration and proper contact, are enforced during the training.   
However, there are several drawbacks of their mesh-based representation for hand-object interaction modeling.
First, they heuristically pre-define regions of the hand that can be in contact with objects.
Second, their object representation is limited to objects of genus zero.
Third, the resolution of their contact inference is limited by the resolutions of the hand and object meshes. 
In contrast, with the grasping field representation, it is not necessary to first compute the hand and object meshes, and then compute the contact region. Instead, one can easily infer the contact region by querying the signed distances of input 3D points. Furthermore, the physical constraints, such as no inter-penetration and proper contact, can be efficiently computed and enforced. 
As demonstrated in our experiments, our model considerably reduces the interpenetration between the reconstructed hand and the object, and improves the quality of 3D hand reconstruction, compared with \cite{hasson2019obman}. 

In summary, our contributions are: (1) We propose the grasping field, a simple and effective representation for hand-object interaction; (2) Based on the grasping field, we present a generative model to yield semantically and physically plausible human grasps given a 3D object point cloud; (3) We further propose deep neutral networks to reconstruct the 3D hand and object given an RGB input in a single pass; (4) We perform extensive experiments to show that our method outperforms the baseline \cite{hasson2019obman} on 3D hand reconstruction and on synthesizing grasps that appear natural.

% \begin{figure*}[th!]
%     \centering
%     % \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
%     \includegraphics[width=0.95\linewidth]{Figure/visual_generated.png}
%     % \vspace{-0.5em}
%     \caption{Ground truth grasps and generated grasps. Each row corresponds to one object. Left three columns show the ground truth grasps, each in three different view points. The middle three columns show one generated example, and the right tree columns show another generated example. Note that these objects are never seen during training. See Appendix~\ref{app:qualitative} (Fig.~\ref{fig:sample}) for more examples.}
%     \label{fig:generative}
% \end{figure*}

%\vspace{-1em}

==> Grasping Field - 3DV/Sec2-RelatedWork.tex <==
\section{Related work}
\label{sec:relatedwork}

% In this section, we first review works that address hand and object pose estimation separately. 
% Then, we discuss the recent works that learn to reconstruct both hand and object jointly.
\textbf{Human grasp and contact.} 
There is a large body of work on capturing and recognizing human grasps \cite{7298666,Glauser:Stretch-Glove:2019,4161001,Nakamura2017,pirk2017understanding,Yang_2015_CVPR}. % as this is highly related to understanding human behavior. Capturing human grasping is an extremely challenging task, as the human hand is highly complex with at least 26 degrees of freedom, not considering soft tissue deformation.
Recently, \cite{Glauser:Stretch-Glove:2019} introduced a stretch-sensing soft glove to capture accurate hand pose without extra optical sensors. Puhlmann et al.~\cite{7759308} utilized a touch screen to facilitate the capturing process of human grasping. As physical contact is fundamental to hand-object interaction, 
%particularly human grasping, 
researchers have proposed methods to capture and modeling contact from diverse modalities \cite{Brahmbhatt_2019_CVPR,2925927}, but these often interfere with natural movement.
Concurrent to this work, \cite{Brahmbhatt_2020_ECCV} proposed a new dataset of hand-object contact paired with RGB-D images.
Our work differs in that our focus is on learning an interaction representation, which is efficient and easy to interface with deep neural networks.

\textbf{Grasp synthesis.} 
Grasp synthesis is a longstanding problem in robotics and graphics, resulting in an extensive literature \cite{AntotsiouImitation,1492758,brahmbhatt2019contactgrasp,siggraph03Handrix,7139730,interactionCaptureSynthesis,4293017, Mahlereaau4984,Iasoniccv2011,Pollard2005, Siggraph91Hans,7138989,6225086,RealtimeHO_ECCV2016,10.1145/2508363.2508412}.
As early as 1991, Rijpkema and Girard \cite{Siggraph91Hans} proposed a knowledge-based approach to incorporate the role of the human hand, object, environment and animator for the task of computer-animated grasping. 
%ElKoura and Singh proposed a data-driven algorithm to model the sympathetic motion between fingers of a human hand and a procedural method to control the fretting hand given a musical passage on a guitar \cite{siggraph03Handrix}.
More recent works can be categorized into three types of approaches: analytic, data-driven and hybrid approaches. For the analytic approaches \cite{Krug2010,6225086}, the grasps are often synthesized by formulating the problem as a constrained optimization problem that satisfies a set of criteria measuring the stability or other properties of the grasps. The data-driven approaches \cite{PintoG16,7139361} often employ machine learning methods to learn representations for synthesizing grasps. An excellent survey of data-driven grasp generation is presented in \cite{10.1109/TRO.2013.2289018}. Recent hybrid approaches \cite{Mahlereaau4984,Mahler2017} combine analytic models and deep learning tools to synthesize grasps for various end effectors. 
Finally, the most related approaches to our work was presented in \cite{corona2020ganhand} and \cite{GRAB2020}, where neural networks are used to predict hand parameters of the MANO hand model \cite{MANO2017} given object information. In \cite{corona2020ganhand}, the model learns to predict the best grasp type from the grasp taxonomy \cite{feix2015grasp} according to the RGB images of the objects. Then, the predicted hands are optimized together with the object meshes to refine the contact points. While in \cite{GRAB2020}, the parameters are generated directly from the given Basis Point Set \cite{prokudin2019efficient} of the objects.
Our work differs from the previous works in that, by also considering the object distance field, we propose a learnable representation for modelling hand-object interaction that can be used without contact post-processing.
Empowered by deep neural networks, the learned representation enables us to synthesize realistic human hand grasping a given object naturally.



\textbf{Hand pose estimation.} 
Hand pose estimation is a long-standing problem, and various input modalities have been considered, e.g., RGB images \cite{baek2020weakly,Doosti_2020_CVPR,Iqbal_2018_ECCV,Mueller_2018_CVPR,8354158,Simon_2017_CVPR,spurr2018cvpr,zimmermann2017learning} or RGB-D and depth sensors \cite{5459282,kerkinECCV12,Malik_2020_CVPR,Mueller2017ICCV,Oberweger_2015_ICCV}.
Due to the lack of large scale 3D ground truth data, synthetic data has often been used for training \cite{Dibra2018a,hasson2019obman,hps2018}.
%These works usually focus on joints estimation and does not provide the complete mesh \cite{...}.
%However, sparse keypoints does not provide enough information to reason about the contact between hand and object.
Recently, instead of estimating the hand skeleton, recovering the pose and the surface of the hand has become popular using statistical hand models, e.g., the MANO model \cite{MANO2017}, that can represent a variety of hand shapes and poses \cite{hampali2020honnotate,Zhang_2019_ICCV,Zimmermann_2019_ICCV}.
Using the template derived from MANO,~\cite{kulon2020weakly} show that it is also possible to regress hand meshes directly using mesh convolution.
%instead to restrict the reconstruction in the valid hand space.
In this work, we represent the 3D hand by a signed distance field, instead of a parametric hand model, due to the difficulty of incorporating object interaction into the model parameter space. For fair comparison with the parametric hand model representation, we fit the MANO model \cite{MANO2017} into our resultant signed distance fields. The experimental results indicate the advantage of our new interaction representation.
%but demonstrate that the MANO model parameters we can be trivially recovered from our reconstruction.

\textbf{Object model representation.} 
Learning 3D object models using various types of representations has also been explored \cite{Chen_2020_CVPR,groueix2018,kato2018renderer,li2016fpnn,Maturana2015iros,michalkiewicz2019deeplevel,PointSet2017,wang2018pixel2mesh,marrnet}.
%\final{Although the use of implicit function for representing shape had been studied before \cite{},}
Recently, the community has focused on using the implicit functions such as the Signed Distance Function (SDF)~\cite{park2019deepsdf}, Occupancy Networks~\cite{mescheder2019occupancy}, Implicit Field~\cite{chen2018implicit_decoder}, and their derivations~\cite{Genova_2020_CVPR,genova2019learning}, as these can model arbitrary object topology with adjustable resolution.
Due to these advantages, we also adopt implicit functions to capture hand-object interaction. %represent object shape as well.
% as it provides the continuous space that makes enforcing contact more efficient and can represent arbitrary shape without object space limitation \cite{park2019deepsdf,mescheder2019occupancy,chen2018implicit_decoder,michalkiewicz2019deeplevel}.

% Using a mesh-based model, however, limits the expressiveness of the model by restricting the possible shape space of the object. Recent works propose the use of implicit function to represent the mesh, which allows the model to represent arbitrary object \cite{park2019deepsdf,mescheder2019occupancy,chen2018implicit_decoder,michalkiewicz2019deeplevel}.
% By deriving implicit representation, we can model arbitrary object. (Also, even though using parametric hand model make it easier for the model to learn, the detail on the surface is still limited by the key points.) (This line will be here only if we get better hand reconstruction result.)

\textbf{Hand-object interaction.} 
Reconstructing hand and object jointly has been studied with both RGB input and RGB-D input \cite{Pham_2018_TPAMI,Rogez:ECCVw:2014,Rogez:CVPR:2015,Romero09,Shan_2020_CVPR,Supancic:ICCV:2015,Tsoli2018,Tzionas:IJCV:2016,Tzionas:ICCV:2015,wang2019learning}.
%Some works(....) focus on contact points using some method(...).
Recently, Hasson~et al. \cite{hasson2020leveraging,hasson2019obman} achieved promising results on explicitly modeling the contact by combining a parametric hand model MANO \cite{MANO2017}, with the mesh based representation for the object. 
As data for hand-object interaction is limited, we opt to use their synthetic dataset, the ObMan dataset \cite{hasson2019obman}, which is sufficiently large for training a neural network. 
%Synthetic data, however, often comes with artifacts like interpenetration, unrealistic contact points, or objects that are not water tight. 
%With our grasping field, we can implicitly manipulate the distance field with an additional loss to have reasonable contact points, thus alleviating the effect of small ground truth artifacts.
Our work differs from previous hand-object reconstruction work mainly by focusing on the novel representation of contact and learning both hand and object in the signed-distance space, which allows arbitrary shape modelling and easier distance field manipulation. Furthermore, we go beyond the reconstruction task by proposing generative models to synthesize realistic human grasps given a 3D object. 

==> Grasping Field - 3DV/Sec3-Method.tex <==
\section{Method}
\label{sec:method}

\subsection{Grasping field}
\label{sec:gf_definition}

The \textit{grasping field} (GF) is based on the signed distance fields of the object and the hand, formally defined as a function $f_{\mathit{GF}}: \mathbb{R}^3 \to \mathbb{R}^2$, mapping a 3D point to the signed distances to the hand surface and the object surface, respectively. In this way, the contact and inter-penetration relations between the hand and the object can be explicitly and efficiently represented. 
Specifically, the hand-object contact manifold is given by $\mathcal{C} = \{\boldsymbol{x} \mid  f_{\mathit{GF}}(\boldsymbol{x}) = \boldsymbol{0} \text{ for } \boldsymbol{x} \in \mathbb{R}^3 \}$. 
The volume of hand-object inter-penetration is given by $\mathcal{I}=\{\boldsymbol{x} \mid f_{\mathit{GF}}(\boldsymbol{x})<\mathbf{0} \text{ for } \boldsymbol{x} \in \mathbb{R}^3 \}$.

Inspired by \cite{park2019deepsdf} and \cite{mescheder2019occupancy}, we propose to model $f_{GF}$ using a deep neural network, and learn it from data. 
Therefore, one can infer hand-object interaction in 3D space without the explicit hand and object surfaces. The learned GF can be considered as an interaction prior, which enables us to infer various grasping poses of the hand, only based on the 3D object.
Furthermore, in contrast to previous works, e.g. \cite{PROX:2019,hasson2019obman,PSI:2019}, which can only evaluate body-object interactions after obtaining the body and the object meshes, when using GF as the representation in hand-object reconstruction from images, we model the hand, the object, and the contact area by the implicit surfaces in a common space, largely improving the physical plausibility of the reconstruction.

According to the aforementioned merits of the GF, we use it to address two tasks in this paper; i.e.~hand grasp generation given 3D objects and hand-object reconstruction from RGB images. Different GF networks are designed specifically for different tasks.



\subsection{Grasping field for human grasp synthesis}
\label{sec:gf_pc}
In this section, we show how to use GF to synthesize human grasps. Given an object point cloud, the goal is to generate diverse hand grasps that interact with the object in a natural manner.

\begin{figure*}[t]
\centering
\subfloat[]{\includegraphics[width=0.65\linewidth]{Figure/GF_pcd_2.png}\label{fig:model_pcd}} 
\vspace{1em}
\subfloat[]{\includegraphics[width=0.25\linewidth]{Figure/hand_seg.png}\label{fig:handLabel}}
\vspace{-1em}
  \caption{(a) Illustration of the generative grasping field network conditioned on an object point cloud. The red dashed arrow denotes sampling from a distribution. Network details are in Appendix~\ref{app:implemmentation}. (b) Illustration of hand part labels. Left is our hand part annotation on the MANO model. Right is an example of our \textit{predicted} surface points with hand part labels. }
\end{figure*}

% \begin{figure*}[t]
% \centering
% \includegraphics[width=0.95\linewidth]{Figure/GF_pcd_2.png}\label{fig:model_pcd}
%   \caption{ Illustration of the generative grasping field network conditioned on the object point cloud. The red dashed arrow denotes sampling from a distribution. Architecture details are described in Appendix~\ref{app:implemmentation}. 
%   }
%   \label{fig:model_pcd}
% \end{figure*}

% \begin{figure}[t]
% \centering
% \includegraphics[width=0.95\linewidth]{Figure/hand_seg.png}\label{fig:handLabel}
%   \caption{Illustration of hand segmentation. Left is our hand part annotation on the MANO model. Right is an example of our \textit{predicted} surface points with hand part labels.}
%   \label{fig:handLabel}
% \end{figure}

% \begin{figure*}[t]
% \centering
% \begin{subfigure}[t]{.7\textwidth}
%     \centering
%     \includegraphics[width=0.9\linewidth]{Figure/GF_pcd_2.png}
%     \caption{}
%     \label{fig:model_pcd}
%     % \vspace{0,5em}
% \end{subfigure}
% \begin{subfigure}[t]{.25\textwidth}
%     \centering
%     \includegraphics[width=\linewidth]{Figure/hand_seg.png}
%     \caption{}
%     \label{fig:handLabel}
% \end{subfigure}
% % \vspace{-1em}
%   \caption{(a) Illustration of the generative grasping field network conditioned on the object point cloud. The red dashed arrow denotes sampling from a distribution. Architecture details are described in Appendix~\ref{app:implemmentation}. (b) Illustration of hand segmentation. Left is our hand part annotation on the MANO model. Right is an example of our \textit{predicted} surface points with hand part labels. }
% \end{figure*}


\paragraph{Network architecture.} The network architecture is shown in Fig.~\ref{fig:model_pcd};
%in which the decoder to produce the grasping field is identical to the one-branch model in Fig. \ref{fig:model_image}. 
we adopt the encoder-decoder framework.
To extract features from point clouds, we use the PointNet encoder \cite{qi2017pointnet} with residual connection. The encoder is trained jointly with other network layers from scratch.
The encoder-decoder network takes a query 3D point, and two point clouds of the hand and the object as input, and produces the signed distances of the query point to the hand and the object surfaces. 
In addition, the encoded object point cloud feature is fed into the hand point cloud encoder, leading to a hand distribution conditioned on the object.
Note that this variational encoder-decoder network only requires both hand and object point clouds during the training. During inference, only the conditioning object point cloud and the query point are required. The hand features are sampled from the learned latent space, as in a standard VAE \cite{kingma2013auto}. 
%\subsubsection{Training loss}
The training loss consists of the following terms:

\myparagraph{The reconstruction loss $\mathcal{L}_{rec}$:} 
For each query point ${\bm x}$, the input object point cloud $p^o$ and the input hand point cloud $p^h$, the reconstruction loss is designed for the hand and object individually: 
%\footnotesize
\begin{multline}
    \mathcal{L}_{rec} = |c(f_{CGF}({\bm x}, p^{o}), \delta ) - c(\text{SDF}_{p^{o}}({\bm x}),\delta )| \\
    + |c(f_{CGF}({\bm x}, p^{h}), \delta ) - c(\text{SDF}_{p^{h}}({\bm x}),\delta )|,
\end{multline}
%\normalsize
where $f_{CGF}$ is the grasping field network (Fig.~\ref{fig:model_pcd}).  $\text{SDF}_{p^{h}}(\cdot)$ and $\text{SDF}_{p^{o}}(\cdot)$ are the ground truth SDF for the hand and object, respectively. In addition,
${c}(s, \delta) := \min (\delta,{max}(-\delta,s))$ is a function to constrain the distance $s$ within $[-\delta, \delta ]$. $\delta$ is set to 1cm in all experiments. 

%Our variational encoder-decoder network is trained using the same reconstruction loss and classification loss as in Eq. \eqref{eq:loss} without the inter-penetration and contact loss. In addition,

\myparagraph{KL-Divergence $\mathcal{L}_{kl}$:} In order to generate new hand grasps, we use a KL-divergence loss to regularize the distribution of hand latent vector $h$, obtained from the hand point cloud encoder $h=E_h(p^h | p^o)$, to be a normal distribution. The loss is given by 
%\scriptsize
\begin{equation}
    \label{eq:loss_kl}
    % \mathcal{L}_{kl} = \textbf{KL-div} \left(N(\mu(p^h | p^o),\sigma(p^h | p^o)) || N(0,{\bm I})  \right),
    \mathcal{L}_{kl} = \textbf{KL-div} \left(N(\mu(h),\sigma(h)) || N(0,{\bm I})  \right),
\end{equation}
%\normalsize
where $N(0,{\bm I})$ denotes a standard high-dimensional normal distribution, $\mu$ and $\sigma$ denotes mean and standard deviation. \
For generation, the hand latent vector $h$ is sampled from a standard normal distribution.
% Such a KL-divergence loss is widely used in the literature.


\myparagraph{Classification loss $\mathcal{L}_{cls}$:}
Besides predicting the signed distances of a query point, we also train the network to produce the hand part label of a query point to parse the hand semantically. To achieve this, we introduce a classification loss, which is given by a standard cross-entropy loss. The hand part annotation is based on the MANO model \cite{MANO2017} as illustrated in Fig.~\ref{fig:handLabel}. 

\subsection{Grasping field for 3D hand-object reconstruction from a single RGB image}
\label{sec:gf_image}

Our proposed grasping field is an expressive representation for modelling hand-object interactions in 3D. 
Here we address the challenging task of 3D hand-object reconstruction from a single RGB image, i.e.~$f_{CGF}: \mathbb{R}^3 \times \mathcal{I} \to \mathbb{R}^2$, in which $I \in \mathcal{I}$ is a 2D image. We model such a conditional GF by two types of deep neural networks and learn their parameters from data.  



\myparagraph{Network architecture.}
The network architectures are illustrated in Fig.~\ref{fig:model_image}, which are designed to recover both hand and object in a single pass. 
%The encoder extracts features from the input image and the decoder produces the grasping field. We use ResNet \cite{he2016deep} as the image encoder, which is pre-trained on ImageNet \cite{russakovsky2015imagenet} and is jointly trained in our experiments.
%The network outputs the SDFs of the hand and the object, respectively. Specifically, the network yields two signed distances from a query point to the closest surfaces of the hand and the object, which appear in the input image. 
To enable a direct comparison with \cite{hasson2019obman}, the two-branch network is employed (Fig.~\ref{fig:two_branch}), which addresses hand and object individually. Similar to \cite{hasson2019obman}, we introduce contact and inter-penetration losses during the training to facilitate a better 3D reconstruction on the contact regions of the hand and the object.
To introduce hand-object interactions in early stages, we propose a one-branch network (Fig.~\ref{fig:one_branch}), which uses the same image encoder and has the same number of layers with the two-branch model. See Appendix~\ref{app:implemmentation} for architecture details.

% \begin{figure*}[t]
% \begin{center}
% \centering
% \subfloat[]{\includegraphics[width=0.5\linewidth]{Figure/two-branch.pdf}\label{fig:two_branch}} 
% \subfloat[]{\includegraphics[width=0.5\linewidth]{Figure/one-branch.pdf}\label{fig:one_branch}}
% \vspace{-0.5em}
%   \caption{Network architectures of the GF conditioned on the image. The blue blocks denote network modules and layers. 
%   A ReLU layer and a dropout layer (dropout ratio 0.2) are between every two consecutive fully-connected (FC) layers. The orange blocks denote feature vectors, and the feature dimensions are presented inside of these feature blocks. The orange dashed boxes denote feature vector concatenation. }
%   \label{fig:model_image}
% \end{center}
% \end{figure*}

% \vspace{-1cm}

% \begin{figure*}[t]
% \begin{center}
% \centering
% % \subfloat[]
% \begin{subfigure}[t]{\linewidth}
%     \centering
%   {\includegraphics[width=0.5\linewidth]{Figure/two-branch.pdf}
%   \caption{}\label{fig:two_branch}}
% \end{subfigure}
% \begin{subfigure}[t]{\linewidth}
%     \centering
%   {\includegraphics[width=0.5\linewidth]{Figure/one-branch.pdf}
%   \caption{}\label{fig:one_branch}}
% \end{subfigure}
% % \vspace{-0.5em}
%   \caption{Network architectures of the GF conditioned on the image. The blue blocks denote network modules and layers. 
%   A ReLU layer and a dropout layer (dropout ratio 0.2) are between every two consecutive fully-connected (FC) layers. The orange blocks denote feature vectors, and the feature dimensions are presented inside of these feature blocks. The orange dashed boxes denote feature vector concatenation. }
%   \label{fig:model_image}
% \end{center}
% \end{figure*}

\begin{figure}[t]
\begin{center}
\centering
\subfloat[]{\includegraphics[width=0.96\linewidth]{Figure/two-branch.pdf}\label{fig:two_branch}} \\
\subfloat[]{\includegraphics[width=0.96\linewidth]{Figure/one-branch.pdf}\label{fig:one_branch}}
\vspace{-0.5em}
  \caption{Two different network architectures of the GF conditioned on the image. The blue blocks denote network modules and layers. 
  A ReLU layer and a dropout layer (dropout ratio 0.2) are between every two consecutive fully-connected (FC) layers. The orange blocks denote feature vectors, and the feature dimensions are presented inside of these feature blocks. The orange dashed boxes denote feature vector concatenation. }
  \label{fig:model_image}
\end{center}
\end{figure}

% \vspace{-1cm}

% Afterwards, the final meshes are obtain by rasterizing the zero level-sets in the estiamted GF via Marching Cubes \cite{marchingcube}.


%\subsubsection{Training loss}Training loss for both the one-branch model and the two-branch model. 
%It comprises %several components and is given by
%\scriptsize
%\begin{equation}
%    \mathcal{L} = \mathcal{L}_{rec} + \alpha_1 \mathcal{L}_{ip} + \alpha_2 \mathcal{L}_{cont} + \alpha_3 \mathcal{L}_{cls}.
%    \label{eq:loss}
%\end{equation}
%\normalsize
%The terms on the rhs of \eqref{eq:loss} correspond to 
%a reconstruction loss, a hand-object inter-penetration loss, a hand-object contact loss, and a classification loss.
\noindent The training loss consists of the following terms:

\myparagraph{The reconstruction loss $\mathcal{L}_{rec}$:} For each query point ${\bm x}$ and the input image $I$, the reconstruction loss is designed for the hand and object individually, and is given by
%\scriptsize
\begin{equation}
    \mathcal{L}_{rec} = \sum_{p \in \{ p^h, p^o \}} |c(f_{CGF}({\bm x}, I), \delta ) - c(\text{SDF}_p({\bm x}),\delta )|,
\end{equation}
%\normalsize
in which $f_{CGF}$ is our conditinal grasping field network, and $\text{SDF}_p(\cdot)$ is the ground truth SDF for the component $p$ (hand or object). ${c}(s, \delta) := \min (\delta,{max}(-\delta,s))$ is the thresholding function to constrain the distance $s$ within $[-\delta, \delta ]$ as with the generative model proposed in Sec.~\ref{sec:gf_pc}.

\myparagraph{The inter-penetration loss $\mathcal{L}_{ip}$:}
To avoid surface inter-penetration between the reconstructed hand and object, we define the inter-penetration loss as
%\scriptsize
\begin{equation}
\mathcal{L}_{ip} = \sum_{{\bm x}} \max ( -\langle {\bm 1},  f_{CGF}({\bm x}, I) \rangle , 0),
\end{equation}
%\normalsize
where ${\bm 1}$ is a 2D one-vector, and $\langle \cdot, \cdot \rangle$ denotes a dot product. This loss function actually penalizes the negative sum of predicted signed distances to the object and to the hand. If the hand and the object are separate and have no contact, the signed distance sum of every point in 3D space is always positive, and hence is ignored by our inter-penetration loss. On the other hand, if the hand and the object have inter-penetration, then this inter-penetration loss does not only penalize the points in the intersection volume, but also all 3D points in the space, indicating that the predicted hand and object are incorrect. 
Compared to the inter-penetration methods in \cite{PROX:2019,PSI:2019}, which only penalize the intersection volume, our loss applies stronger constraints.


\myparagraph{Contact loss $\mathcal{L}_{cont}$:}
Our proposed contact loss encourages hand-object contact, and is given by 
%\scriptsize
\begin{equation}
\mathcal{L}_C = \sum_{\bm x}{\min}(\alpha |f_{CGF}({\bm x}, I)|^2, 1),
\end{equation}
%\normalsize
where $\alpha$ is a hyper-parameter. 
We can see that $f_{CGF}({\bm x}, I)=0$ corresponds to the hand-object contact surface. Therefore, it ignores points with predicted grasping field $ |f_{CGF}({\bm x}, I)|^2 \geq \frac{1}{\alpha}$, and only encourages points with $ |f_{CGF}({\bm x}, I)|^2 < \frac{1}{\alpha}$ to be the contact points. In our study, we empirically set $\alpha=0.005$ based on the hand-object interactions in the training data.
Finally, we employ the same \textbf{Classification loss $\mathcal{L}_{cls}$} as the one proposed in Sec.~\ref{sec:gf_pc}.


%%%


\subsection{From grasping field to mesh}
\label{subsec:fromGF2Mesh}
With the trained grasping field conditioned on images or point clouds, one can compute the signed distances to the hand and object of a query 3D point. To recover the hand, object and their interactions, we first randomly sample a large number of points, and evaluate their signed distances. The point clouds belonging to the hand and the object can be selected, according to point-object signed distances close to zero. Then, the hand mesh and the object mesh are obtain by marching cubes \cite{marchingcube}.

In addition, the hand mesh can be recovered by fitting the MANO  \cite{MANO2017} model to the hand point cloud. In this case, we can obtain hand segmentation, hand joint positions, and a compact representation of the hand simultaneously, according to the pre-defined topology in MANO. 

Denoting the MANO model by $\mathcal{M}(\beta, \theta)$ with the parameter $\beta$ and $\theta$ representing hand shape and pose respectively, we minimize 
$\sum_{l=1}^{6} d(\tilde{p}^h, \mathcal{M}(\beta, \theta)^l)$ 
% \scriptsize
% \begin{equation}
%     \mathcal{L}_{MANO} =
%     \min_{\beta, \theta} \sum_{l=1}^{6} d(\tilde{p}^h, \mathcal{M}(\beta, \theta)^l)
% \end{equation}
%\normalsize
to recover the hand configuration, in which $l$ denotes the 6 parts of hand, i.e. the palm and the 5 fingers, $\tilde{p}^h$ denotes the hand point cloud produced by our model, $\mathcal{M}(\beta, \theta)^l$ denotes the MANO hand mesh belonging to the hand part $l$, and $d(\cdot, \cdot)$ denotes the Chamfer distance \cite{fan2017point,park2019deepsdf}. The hand segmentation is shown in Fig. ~\ref{fig:handLabel}.

The implementation details are thoroughly presented in Appendix~\ref{app:implemmentation}.
 




% \newpage
% \section{Method-bk}

% \begin{figure}
% \begin{center}
% \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
%   \caption{[Placeholder] Our model}
%   \label{fig:model}
% \end{center}

% \end{figure}

% Our neural network architecture is designed to reconstruct both hand and object in a single pass. We adopt the encoder-decoder framework where the encoder learn a meaningful latent code from an image and then the decoder learn to represent that latent code with a signed distance function.
% The network is split into two branches of decoders, one for representing the signed distance function to the hand surface, the other to the object surface.
% The encoder can be changed depending on the task.

% The final mesh is obtain by rasterizing the zero-level surface using Marching Cubes \cite{marchingcube}.
% The overview of our model is shown in Figure \ref{fig:model}.

% In the following, we provide the details of both component and motivate the use of signed distance function to jointly learn to reconstruct hand and object.






% % ----------------- SDF -------------------
% \subsection{Signed distance function (SDF)}
% \textcolor{blue}{comment Jinlong: I think there's too much text for sdf}
% Using an implicit function to represent object surface instead of mesh was proposed by many recent works \cite{park2019deepsdf}. We adopt a deep signed distance function \cite{park2019deepsdf} as a method for representing hand and object surface in our model as it enable a natural way for the model to reason about contact. A signed distance function is a function that output the distance from a query point to the closest surface, with a sign to indicated whether a point is inside or outside of the watertight mesh.

% % signed distance function
% % latent space of hand shape and object shape

% In our task, as we want to reconstruct hand and object from an encoded image, the SDF decoder is condition on the encoded vector $z_i$ and the query point $x$:

% \begin{equation}
% f_\theta(z_i, x) \approx {SDF}^i(x)
% \end{equation}

% Following DeepSDF \cite{park2019deepsdf}, we train the decoder using $L_1$ loss function with clamp parameter $\delta$:
% \begin{equation}
% \mathcal{L}( f_\theta(x),s) = |{clamp}(f_\theta(x),\delta) - {clamp}(s,\delta)|
% \end{equation}
% where ${clamp}(x, \theta) := {min}(\delta,{max}(-\delta,x))$ constrains the distance from the surface we want the network to pay attention to. In our setting, $\delta$ is set to 1cm for all experiments.

% In order to train the decoders as approximators of signed distance function, for each input image, a single latent code is obtained from the encoder, then the 3D position of point $p$ is concatenated to the latent code and passed to the decoder. The decoder then learn to predict the signed distance between the given point and the mesh surface.
% The reconstructed mesh can be obtained by discretization of this space and extract the zero-level surface using Marching Cubes.

% % \textcolor{red}{KRIK: I would suggest to put this section a bit earlier. It is our main methodology.}

% % To reconstruct the object mesh, we used a neural network to learn a signed distance function conditioning on the encoded RGB image and a given point in 3D space. We then derived the mesh by finding a zero-valued iso-surface using Marching Cube~\cite{marchingCube}. (cite DeepSDF~\cite{park2019deepsdf}).

% By using implicit function to represent object in this task, our network is not constrain to output only genus 0 topologies and can learn to represent any arbitrary object.\textcolor{blue}{comment Jinlong: Save this for now but we need to show example}



% \subsection{Jointly learn SDF for hand and object}
% In order to reconstruct a meaningful hand-object interaction, the two function are needed to be learn together. 
% Instead of using parametric hand model (e.g MANO \cite{MANO2017}), we observe that by viewing both hand and object reconstruction as an optimization in SDF space, the contact can be enforced by regularize the predicted distance to comply with some simple conditions. 
% Here, we formulate these conditions as a differentiable loss , $\mathcal{L}_{Interaction}$, which can be use as a regularization term for end-to-end learning.
% We aim to formalize two specific circumstances that govern the basic conditions of interaction between hand and object, interpenetration and contact.

% % For a point sampled from the 

% % interpenetration
% \subsubsection{Interpenetration}
% As the reconstruction hand and object should not overlap with each other, we define the interpenetration loss term to prevent the model to make unrealistic prediction. The interpenetration loss $\mathcal{L}_{I}$ is define as:

% \begin{equation}
% \mathcal{L}_I = \sum_{p_i} {max}(-(S_h(p_i) + S_o(p_i)), 0)
% \end{equation}
% where $S_h(p_i)$ and $S_o(p_i)$ are predicted signed distances to hand and object mesh of a sample point $p_i$.

% When there is interpenetration between meshes, one of the following cases will be true: (i) $S_h(p_i) < 0$ and $S_o(p_i)<0$, or (ii) if $S_h(p_i)<0$ or $S_o(p_i)<0$, $-{min}(S_h(p_i),S_o(p_i)) > {max}(S_h(p_i),S_o(p_i))$.
% For any spatial point, this $\mathcal{L}_I$ will penalize those cases.
% % distance from a given point to the closest surface on the hand mesh and the closest surface on the object mesh.

% % Each pair of hand and object mesh is normalized into a unit cube


% \subsubsection{Contact}
% The basic condition for hand-object interaction is that the two mesh should be in contact with each other. We design the contact loss such that it will generate gradient to pull the surface of hand and object together if the two mesh are close and generate no gradient otherwise. In the same way as interpenetration loss, the value is calculated in the canonical space which allows the loss weight to have a meaning in the canonical space. Specifically, for a point in 3D space, how much distance should the model compromise to make the contact.
% The contact loss $\mathcal{L}_{C}$ is define as:

% \begin{equation}
% \mathcal{L}_C = \sum_{p_i}{min}(\alpha (S_h(p_i)^2 + S_o(p_i)^2), 1)
% \end{equation}

% This loss term can be viewed as a tunable trade-off between enforcing the model shape and enforcing contact.

% \subsubsection{Combining the two losses}
% As the two losses do not directly interfere with each other, Their weights can be tune separately to maintain their meaning in canonical space. We define $\lambda_I$ and $\lambda_C$ as weight for the interpenetration loss and contact loss, respectively.
% The model is then trained with the following loss term:

% \begin{equation}
% \mathcal{L} = \mathcal{L}_{R} + \lambda_I \mathcal{L}_{I} + \lambda_C \mathcal{L}_{R}
% \end{equation}
% where $\lambda_I$ and $\lambda_C$ is set to 1.0(...cm) and 15.0(...cm) in our setting.
% By defining these losses in the canonical space, we allow the interpretable trade-off of reconstruction loss allowed to make contact.


% % --------------------------------------------------------------------
% \subsection{MANO from reconstructed hand mesh} \label{manoFitting}

% \begin{figure}
% \begin{center}
% \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
% %   \includegraphics[width=0.6\linewidth]{Figure/m2m_dist.png}
%   \caption{[Placeholder] Hand label reference mesh and prediction}
% \end{center}
% \label{fig:handLabel}
% \end{figure}


% Though we show that the DeepSDF can learn to reconstruct hand mesh in a non-parametric manner, hand joints location are still useful for certain tasks. In this subsection, we demonstrate a way to obtain the parameters for hand model MANO by modifying a part of our model. To achieve this, we add a new objective to the trained model, predicting which part of a hand each spatial point belongs to. 
% We designed a label assignment that separates the palm and each finger from each other, resulting in 6 possible labels (Fig \ref{Fig:handLabel}).
% With the reference mesh, the ground truth label for each training point can be obtained together with the SDF value during the sampling. For each point, the label means which part of the hand its closest point on the surface belongs to.
% Adding the new classification loss, $\mathcal{L}_{L}$, the loss function of our network now becomes:

% \begin{equation}
% \mathcal{L} = \mathcal{L}_{H} + \mathcal{L}_{O} + \lambda_L \mathcal{L}_{L}
% \end{equation}
% where the weight for the label classification loss, $\lambda_L$, is set to 0.1 throughout the training.


% Using these labels, we can optimize the reference MANO mesh to match the labels at the zero-level surface of our prediction using the differentiable MANOLayer \cite{hasson2019obman}. The optimization can be expressed as:

% % need the equation here ....
% \begin{equation}
% E = \arg\min_{\theta, \beta}\sum_{l = 0}^6 d(\bm{v}_l, \bm{p}_l) 
% \end{equation}
% where $\theta$ and $\beta$ are MANO pose and shape parameters respectively; $\bm{v}_l$ and $\bm{p}_l$ are MANO vertices and reconstructed hand surface points with hand part label $l$; $d(,)$ denotes Chamfer distance between two point could.


% %-------------------------------------------------------------------------
% %%%%%%%%% Implementation Details
% \subsection{Implementation Details}
% As the Grasping Field model learn to generate shape from the latent code, the encoder can be changed depending on the tasks. 
% For single image reconstruction, we use a Resnet18 \cite{he2016deep} pretrained on ImageNet dataset \cite{russakovsky2015imagenet} as an encoder. 
% For point cloud input, we use a variation of PointNet encoder \cite{qi2017pointnet} with residual connection provided by \cite{mescheder2019occupancy}. Unlike for image input, we use two identical encoder to process hand and object point cloud. The two latent code are concatenated before going in to the decoder.

% For conditional hand generation, we use the same object encoder to compute object latent code, $z_{obj}$. The hand encoder take hand point cloud $p_i$ and object latent code $z_{obj}$ as input, then predict mean $\mu$ and standard deviation $\sigma$ of a Gaussian distribution $q_{\psi}(z_{hand}|p_{i=1:K},z_{obj})$ on the hand latent $z_{hand}$.
% We condition the hand encoder on object latent code $z_{obj}$ by concatenating $z_{obj}$ to the output of each point from the first layer.
% We optimize the lower bound \cite{kingma2013auto,rezende2014stochastic} of the KL term defined as:

% \begin{align}
%   \mathcal{L}_{KL} & = KL(q_{\psi}(z_{hand}|p_{i=1:K},z_{obj}) || p_0(z_{hand}))
% \end{align}
% where $KL$ is the KL-divergence, $p_0(z_{hand})$ is a Gaussian prior on the latent code $z_{hand}$.

% As we observe that the decoder cannot learn to interpret the latent code in a signed distance function space if the KL loss term is introduced too early, we train the first 200 epochs with the weight $\lambda_{KL}$ set to zero. The weight is then linearly increased to 0.1 over the next 200 epoch \cite{bowman2015generating}.

% During training, we randomly selected half of the training points $p_i$ from point sample around the hand mesh and the other half from the object mesh.
% The L1-loss generated with respect to the distance the other mesh (hand point to object surface/object point to hand surface) is masked out until the contact loss is later introduced into the training.
% We observe clear degradation when training without this mask as the sampled points are bias toward the region that is closer to the other mesh.


==> Grasping Field - 3DV/Sec4-Experiments.tex <==
\begin{figure*}[t!]
\centering
\includegraphics[width=1.0\linewidth]{Figure/sample_HO3D_full_col.png}
  \caption{Generated grasps conditioned on objects from the HO3D dataset. Each pair shows the sampled grasp from two viewpoints. The model is trained only on the ObMan \cite{hasson2019obman} dataset.}
  \label{fig:sample_ho3d_main}
\end{figure*}

\section{Experiments}
\label{sec:experiments}
% \setlength{\textfloatsep}{5pt}

We demonstrate the effectiveness of the grasping field representation on two challenging tasks: human grasp generation given a 3D object and 3D hand-object reconstruction from a single image.  
%By evaluating on the \textbf{hand-object reconstruction} from a RGB image, we show that the learned grasping field is an effective representation for hand-object interaction, and is able to recover 3D shapes of the hand and the  object effectively. More importantly, we show that by employing the novel interaction representation, we are able to considerably improve the reconstruction quality in terms of the physical plausibility. 
%In the second experiment, we validate our approach in a \textbf{generative setting}, where we evaluate the semantic and physical plausibility of the proposed generative model given only the 3D object point cloud as input. 


\paragraph{Dataset.}
To train the generative model for human grasp synthesis, we need ground truth 3D meshes of interacting hands and objects. Unfortunately,  existing datasets often lack the desired properties.% \cite{zimmermann2019freihand}. 
The limitations include small dataset size and lack of 3D ground truth hand pose or shape. %only key-points for hand shape. %or having limited variation of manipulated objects.
Consequently we use the synthetic \textbf{ObMan dataset}~\cite{hasson2019obman} to train our model. 
%It contains synthetic 3D meshes for both hand and object and rendered images. 
The data is generated from a statistical hand model, MANO \cite{MANO2017}, and 2772 object meshes covering 8 classes of everyday objects from the ShapeNet dataset~\cite{chang2015shapenet}.
Hand-object interaction is generated using a physics simulator, GraspIt~\cite{miller2004graspit}, resulting in high-quality hand-object interaction. 
%We follow the method provided by Park et al.~\cite{park2019deepsdf} to remove small portion of the dataset with problematic object meshes and finally form a training set of 86,058 samples and test set of 3,884.
Due to the limited number of grasp types in the \textbf{FHB dataset} \cite{garcia2018fhb} and the \textbf{HO-3D dataset} \cite{hampali2020honnotate}, they are not suitable for training the generative model (see Appendix~\ref{app_dataset_analysis}). 
Instead, we use them to test the generalization ability of the generative model trained on the \textbf{ObMan} grasps. 

For the 3D reconstruction task, we also mainly use the \textbf{ObMan dataset} for training and testing. To test the effectiveness of our network on real-world images, however, we follow the same approach as \cite{hasson20_handobjectconsist} to train and test on the \textbf{FHB dataset}. 

\paragraph{Evaluation metrics.}
Our goal is to generate physically plausible and semantically meaningful 3D human hand given an object. Therefore, 
we quantitatively evaluate the generated samples according to physics-based metrics and use large-scale perceptual studies to measure the visual realism of the grasps. For the 3D reconstruction task, we use Chamfer distance and hand joint error. Details of the evaluation metrics are in Appendix~\ref{app:eval_metrics}.

\textbf{(1) Physical metrics:} A valid human grasp implies stable hand-object contact without interpenetration. Consequently, we use the following evaluation metrics:
\textit{\textbf{a) Intersection volume and depth}}. The hand and object mesh are voxelized and the interpenetration depth is the maximum distance from all the intersected voxels to the surface of another mesh. \textit{\textbf{b) Ratio of samples with contact}}. We define a \textit{contact} between the object and the hand when any point on the surface of the hand is on or inside the surface of the object. We calculate the ratio of samples over the entire dataset that have interpenetration depth more than zero.
\textit{\textbf{c) Grasp stability}}. Using physics simulation \cite{coumans2013bullet}, we hold the hand constant, apply gravity, and measure the average displacement of the object's center of mass during a fixed time period. 
%Small displacement suggests a stable grasp.

\textbf{(2) Semantic metric:} We perform perceptual studies using Amazon Mechanical Turk to evaluate the naturalness of our generated grasps. Details of the study are presented in Appendix~\ref{app:eval_metrics} and~\ref{app:user_study}.

\textbf{(3) 3D reconstruction quality:} We use the Chamfer distance between reconstructed and ground truth hand surfaces to evaluate the hand reconstruction quality as in~\cite{park2019deepsdf}.
Hand joint distance is computed following \cite{hasson2019obman,zimmermann2017learning}.


\begin{table*}[t]
    \centering
    % \scriptsize
    \caption{Evaluation of the grasp synthesis on the objects from the ObMan test set, FHB and HO3D. GT* indicates that the ground truth grasps are obtained by fitting the MANO model to the data. Best results except the ground truth are shown in boldface. }
    % \vspace{-1em}
    %\begin{tabular}{p{30pt} p{12pt}p{12pt}p{12pt}p{12pt}p{12pt}| p{12pt}p{12pt}p{12pt}p{12pt}p{12pt} |p{12pt}p{12pt}p{12pt}p{12pt}p{12pt}}
   \begin{tabular}{l c c c | c c c | c c c}
    \toprule
        &  \multicolumn{3}{c} {\bf ObMan}  &  \multicolumn{3}{c} {\bf FHB}    &  \multicolumn{3}{c}{\bf HO3D}\\
        & GT &  Baseline & GF   & GT*  &   Baseline & GF  & GT & Baseline & GF \\
        \midrule
        Contact ratio ($\%$) $\uparrow$      & - & 66.89 & \bf{89.4} &92.2 & 48.8& \bf{97.0}  & 93 &  44.3& \bf{90.1}\\
        Intersection vol. ($cm^3$) $\downarrow$ & - & 14.46 & \bf{6.05}  &16.6& \bf{9.65} & 21.9  & 10.5& \bf{5.86} &14.9\\
        Intersection depth ($cm$) $\downarrow$  & - & 0.94  & \bf{0.56}  & 1.99 & \bf{1.77} & 2.37 & 1.47 & \bf{1.01} &1.46\\
        Physics simulation ($cm$) $\downarrow$   &1.66  & 4.56  & \bf{2.07}  &6.69  & 8.59   & \bf{4.62} & 4.31  &8.25 & \bf{3.45} \\   
        & $\pm$ 2.42 & $\pm$ 4.57 & $\pm$ 2.81 & $\pm$ 5.48 & $\pm$ 3.67 & $\pm$ 4.48 & $\pm$ 4.42 & $\pm$ 4.18 & $\pm$ 3.92 \\
        Perceptual score $\{1...5\}$ $\uparrow$   & 3.24  & 2.40  & \bf{3.02}  & 3.49 & 2.43 & \bf{3.33} & 3.18 & 2.03 & \bf{3.29}\\
    \bottomrule
    \end{tabular}
    \label{tab:generation_model_full}
\end{table*}



\subsection{Evaluation: Human grasps generation}
\label{sec:eval:generation}
%We analyze the representation power of the grasping field for human grasp synthesis in this section.

\myparagraph{Baseline.} To our knowledge, there is no previous model that learns to synthesize natural human grasps given a 3D object. Rather than randomly placing the hand around the object, we trained a strong baseline model for grasp generation. Specifically, we replace the decoder (i.e.~the grasping field) of our conditional VAE model (Fig.~\ref{fig:model_pcd}) with fully connected layers to regress MANO hand parameters. Then given a 3D object point cloud and a random sample, our baseline model generates MANO parameters directly. Generated grasps from the baseline are shown in Appendix~\ref{app:qualitative}. 
%We believe our baseline model enables valid analysis and comparison, as the network architecture is of common practice and the generated grasps are sensible. 



\myparagraph{Results.} We show the systematic quantitative evaluation of the generative method in Tab.~\ref{tab:generation_model_full} and qualitative results in Fig.~\ref{fig:generative},~\ref{fig:sample_ho3d_main} and Appendix~\ref{app:qualitative} (Fig.~\ref{fig:sample},~\ref{fig:sample_ho3d}). The baseline and the GF model are only trained on the \textbf{ObMan} training set, and tested extensively on the objects from the \textbf{ObMan} test set, \textbf{FHB} and \textbf{HO3D}. Our proposed GF performs substantially better than the baseline on \textbf{ObMan} and achieves comparable quality as the ground truth grasps. 
%Though only trained on ObMan dataset, our model generate similar quality of grasps on FHB and HO3D dataset as the ground truth. 
When the model is tested on the \textbf{FHB} objects, which are never seen during training, it achieves a comparable perceptual score compared to the ground truth grasps. 
%\textcolor{red}{Unclear: On \textbf{HO3D}, our synthesized grasps even outperform the ground truth grasps (3.29 vs 3.18). Note that the ground truth are obtained from human grasps. }
Surprisingly, on \textbf{HO3D}, our synthesized grasps are judged more realistic than the ground truth grasps of real humans (3.29 vs 3.18).
These perceptual studies suggest that our method makes an important step towards the fully automatic synthesis of realistic human grasps. 

Regarding the physical plausibility, we observe that our model achieves a better contact ratio and grasp stability (physics simulation) than the ground truth grasps on \textbf{FHB} and \textbf{HO3D}. 
This is likely due to the GF results having a larger intersection volume.
One reason is that there are a very limited number of objects in these two datasets.
Some of the test objects are very different from the training objects, resulting in more inter-penetration for the generated grasps.
Overall, the combination of visual realism and grasp stability suggests that our results are approaching the level of natural human grasps.

%Overall, we argue that the generated grasps archive a comparable performance on the unseen objects, comparing to the ground truth grasps provided by the datasets that capture real human grasps. 

%on The perceptual quality is significantly improved by our model compared with the baseline method. We visualize some random samples from the result in Figure~\ref{fig:result_generation}
% The generation quality is comprehensively analysed with 5 different metrics. \textcolor{red}{discussion of the results needs to be added when the numbers are there.} 

%On the Obman testset, our model consistently outperforms the baseline for the physics and semantic metrics. 

\setlength{\tabcolsep}{4pt}
\begin{table*} [t!]
% \scriptsize
\caption{3D reconstruction results on \textbf{ObMan} (a) and \textbf{FHB} (b). 
%GF-MANO indicates the results after substituting implicit hand surface with recovered MANO meshes;
2De refers to the 2 decoder model; 
L indicates the corresponding model is trained with the contact and interpenetration loss; GF-MANO refers to the MANO hand obtained by fitting the MANO model to the SDF.
}
\begin{minipage}{.7\linewidth}
\centering
\begin{tabular}{l|ll|l|ll|l|ll}
% \hline\noalign{\smallskip}
\toprule
Models  & \multicolumn{2}{l}{Hand error} & Joints & \multicolumn{2}{l}{Intersection} & Contact  & \multicolumn{2}{l}{Object Error} \\
 & Mean & Med  & (cm) & Vol & Depth & (\%)  & Mean & Med\\

% \noalign{\smallskip}
\midrule
GF   & 0.419 & 0.283 & - & 0.65 & 0.32 & 90.8  & 12.8 & 6.4 \\
GF+L & 0.400 & 0.261 & - & 0.00 & 0.00 & 5.63  & 14.2 & 6.8\\
%GF+L-MANO & - & - & 0.415 & 0.280 & 0.11 & 0.07 & 28.67 & 0.01 \\
GF-2De  & 0.408 & 0.262 & - & 8.56 & 1.01 & 99.6 & 11.1 & 5.7\\
GF-2De+L& 0.384 & 0.237 & - & 0.23 & 0.20 & 69.6  & 11.7 & 5.9 \\
%GF-2De+L-MANO & - & - & 0.406 & 0.277 & 0.16 & 0.13 & 52.26 & 1.13 \\

\midrule

GF-MANO  & 0.405 & 0.272 & 1.13 & 0.59 & 0.27 & 83.3  & - & - \\
GF-2De-MANO & 0.419 & 0.276 &  1.14 & 5.75 & 0.87 & 98.9 & - & - \\
\midrule
Hasson et al.~\cite{hasson2019obman}  & 0.533 & 0.415 & 1.13 & 6.25 & 1.20 & 94.8  & 6.7 & 3.6 \\
\bottomrule
\end{tabular}
% \vspace{-1em}
\captionsetup{labelformat=empty}
\caption{(a)}
\end{minipage}
\begin{minipage}{.2\linewidth}
\begin{center}
\begin{tabular}{l c}
\toprule
Models & Hand Joints \\ 
 & (cm) \\
\midrule
GF-MANO\\(MANO joints) & 2.60\\
\midrule
GF-MANO \\(FHB marker) & 2.94\\
\midrule
Hasson et al.*~\cite{hasson20_handobjectconsist} & 2.74\\
\bottomrule
\end{tabular}
% \vspace{-1em}
\captionsetup{labelformat=empty}
\caption{(b)}
\end{center}
\end{minipage}
\label{table:imageResults}
\end{table*}


\subsection{Evaluation: 3D hand-object reconstruction } \label{subsec:result_image_condition_v2}
Apart from serving as a powerful representation for the synthesis task, the proposed GF also facilitates the 3D reconstruction task.
In the following, we analyze the different network architectures and training losses proposed in Sec.~\ref{sec:gf_image}. We compare with the baseline method~\cite{hasson2019obman} on the \textbf{ObMan} dataset and  \cite{hasson20_handobjectconsist} on the \textbf{FHB} dataset. The results are summarized in Tab.~\ref{table:imageResults}. Due to many limiting factors of the real-world datasets such as \textbf{FHB} and \textbf{HO3D} (see Appendix~\ref{app_dataset_analysis} for detailed data analysis), learning a reasonable model for joint object and hand reconstruction is extremely challenging. Instead, to evaluate the effectiveness of the GF representation for 3D reconstruction on real-world images, we follow the setting of the latest work \cite{hasson20_handobjectconsist}, where the object 3D model is given as input. Note that this is a commonly used setting in previous works (e.g.~ \cite{hasson20_handobjectconsist,kehl2017ssd,Tekin_2019_CVPR}).
%We train and evaluate the 3D reconstruction network on the ObMan dataset.
%Result in Table~\ref{table:imageResults} shows that our model achieves comparable performance as the state of the art.

\myparagraph{Network design.}
We first analyze the two different network architectures presented in Fig.~\ref{fig:model_image} denoted with and without `2De' respectively. 
%The results from the two-branch-decoder design are denoted by ``2De''. 
Both architectures achieve comparable performance for hand reconstruction, however differ significantly for intersection error, where the one decoder model achieves considerably better performance, due to the efficient joint modeling of hand-object interaction. Compared with the baseline \cite{hasson2019obman}, the intersection volume and depth are reduced from 6.25 and 1.20 to 0.65 and 0.32, respectively. The contact ratio are comparable among two architectures and baseline model.
All our models considerably improve the quality of hand reconstruction, compared with \cite{hasson2019obman}. The object reconstruction quality is behind hand quality for all model variations including the baseline model. 
Note that the \textbf{ObMan} dataset contains more than 1600 objects from 8 different classes. The object reconstruction performance is decreased as it remains unclear how to learn the implicit representations to reconstruct a large variety of object classes with a single model \cite{mescheder2019occupancy,park2019deepsdf} and such a task is beyond the focus of this work.  
%This is caused by large object shape variation, heavy occlusion and low image quality. 
Please see Appendix \ref{app:qualitative} (Fig.~\ref{fig:recon}) for visualization.

% \textcolor{red}{The rest of this is confusing:
% Although the contact percentage decreases from 94.8 to 90.8, the overall reconstruction quality of the physical plausibility is largely improved by our approach. All the models considerably improve the quality of hand reconstruction. 
% Note that the ObMan dataset contains more than 1600 objects from 8 different classes. The object reconstruction performance is decreased as it remains unclear how to learn the implicit representations to reconstruct a large variety of object classes with a single model \cite{mescheder2019occupancy,park2019deepsdf} and such a task is beyond the focus of this work.   
% }

\myparagraph{Training losses.}
The effect of the contact and interpenetration loss ($+$L) is shown in Tab.~\ref{table:imageResults} (a), 
when the loss is imposed during the training of the two-decoder network, the intersection volume and depth are reduced and the overall quality of the interaction is considerably improved. In contrast, for the one-decoder model, our observation is that, for a large portion of 3D points, the signed distances to the object and to the hand are highly correlated, the model that jointly predicts both signed distance values does not need to enforce this auxiliary training loss.

%and decreases the performance of object reconstruction, comparing to the baseline model \cite{hasson2019obman}. Our observation is that the learned distance function has difficulties to reconstruct a large variety of objects. 

%We observe that for a large portion of 3D points in the space, the signed distance of object and the one of hand are highly correlated. Based on this observation we propose GF to model them together. As a result, a single neural network that jointly predicts both signed distance values should be more efficient than a two-decoder model of the same network size. Table~\ref{table:imageResults} proves this by showing a clear boost of proposed model over a two-decoder model on intersection depth and contact. Figure~\ref{fig:contactCurve} better visualizes the improvement.

%\myparagraph{Contact and interpenetration losses.}
%For two-decoder model, since object and hand correlation is not modeled together, adding extra contact and interpenetration loss can strongly improve the contact quality as shown in Table~\ref{table:imageResults} and Figure~\ref{fig:contactCurve}. But proposed GF models the joint distribution of hand and object, such that this extra supervision is no longer necessary as shown in the curve.

\myparagraph{MANO fitting.}
As shown in Tab.~\ref{table:imageResults} (a), MANO fitting (indicated by GF-MANO) does not have a substantial influence on the reconstruction quality. This implies that on the one hand, the reconstructed hand of our GF model is realistic enough without a statistical model to regularize it, and that on the other hand, the output hand part labels are accurate enough for us to fit the MANO model and retrieve hand joints or shape parameters for applications that need these without undermining the shape and contact estimation.
A qualitative illustration is presented in Fig.~\ref{fig:mano_fit}.

%We show a few samples of our reconstruction result in Figure~\ref{fig:imageResults}, more examples can be found in the supplemental material.

\myparagraph{Hand reconstruction on real-world images.} 
To analyse the effectiveness of the proposed grasping field representation for the 3D reconstruction task on real-world images, we compare our method with the latest work \cite{hasson20_handobjectconsist} on the \textbf{FHB} dataset. Compared to \cite{hasson2019obman}, the key difference in~\cite{hasson20_handobjectconsist} is that the object is given as part of the input. We explore the same network architecture as \cite{hasson20_handobjectconsist} and only replace the decoder part with the grasping field.
The implementation details are presented in Appendix~\ref{app:implemmentation} (Fig.~\ref{fig:network_object_input}).
%(See Appendix~\ref{app:implemmentation} (Fig.~\ref{fig:network_object_input}) for the implementation details). 
% In order to train our model on the \textbf{FHB} dataset, we fit the MANO model to obtain the pseudo ground truth of the hand SDF.  

As stated in \cite{hasson20_handobjectconsist}, definition of hand joint locations vary between datasets. 
Without hand surface annotation in the FHB dataset,
%which contains images of human hand interacting with objects, 
it is difficult to train an accurate regressor that maps between the FHB markers and the MANO joints. Assuming that the joints are identically defined, we fit the MANO model to the FHB markers by minimizing the distance between the MANO joints and the FHB markers. Then the MANO joints obtained in such way are considered as our pseudo ground truth joints, and the obtained MANO surface  is used to supervise the training. 

We compare the predicted MANO joints with the pseudo ground truth joints as well as the original FHB markers assuming identical joints. 
% Hasson et al. compares their model output against the FHB markers.
% The defined locations for the FHB dataset do not match the MANO joints. Meanwhile, our training objective is the MANO surface and our model can not optimize for the FHB joints.
As our model is not trained to optimise for the FHB marker locations, the reconstruction error is larger than~\cite{hasson20_handobjectconsist} as shown in Tab.~\ref{table:imageResults} (b). When we evaluate our prediction on the pseudo ground truth MANO joints, the reconstruction error decreases from $2.94 cm$ to $2.6 cm$. This suggests that the proposed grasping field representation is effective for the task of 3D hand reconstruction from a single image, achieving comparable performance with respect to the start-of-the-art. 




%In contrast, the grasping field is able to reconstruct the better hand surface comparing to \cite{hasson2019obman}, 
%Table~\ref{table:imageResults} summarizes the evaluation of our method on hand-object reconstruction task and comparison with baseline method Hasson et al.~\cite{hasson2019obman}. 
%We found that our model can predict reasonable hand surface with high contact quality. Our method has overall better performance on hand reconstruction and contact estimation with respect to Hasson et al.~\cite{hasson2019obman}. On object shape reconstruction, neither method achieves satisfying result. It is caused mainly by large object shape variation and strong object occlusion from single image.
% After the fitting MANO model to implicit hand surface, the hand Chamfer distance show improvement on ObMan dataset.From joints evaluation, We note the comparison of joint error and hand chamfer distance between our model and \cite{hasson2019obman}. Our model could achieve better Chamfer distance while having almost identical joint error. This suggest that when optimizing MANO pose and shape parameter there might be a few combinations which generate relatively low joint error but differ greatly from each other. 

%\begin{figure}
%\begin{center}
%% \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
%  \includegraphics[width=0.6\linewidth]{Figure/m2m_dist.png}
%  \caption{[Cumulative ratio of interpenetration distance over ObMan dataset \textcolor{blue}{Todo: 1. Replace the curve with latest result. 2. add an ideal curve; 3. Change the axis label or text for that they match each other}}
%\end{center}
%\label{fig:contactCurve}
%\end{figure}



%\begin{figure}
%    \centering
%    \includegraphics[width=0.9\linewidth]{Figure/visual_reconstruction.png}
%    \caption{Qualitative result of image conditioned model. From left to right: test image, predicted implicit hand and object surfaces in two different view points, MANO fitted hand prediction, ground truth hand and object.}
%    \label{fig:imageResults}
%\end{figure}{}

==> Grasping Field - 3DV/Sec5-Conclusion.tex <==
\section{Conclusion and Discussion}
\label{sec:conclusion}

In this work, we propose a novel representation for hand-object interaction, namely the grasping field. 
Learning from data, the GF captures the critical interactions between hand and object by modeling the joint distribution of hand and object shape in a common framework.
To verify the effectiveness, we address two challenging tasks: human grasp generation given a 3D object and shape reconstruction given a single RGB image. The experiments show that the generated hand grasps appear natural and are physically plausible while the hand reconstruction achieves comparable performance as the state-of-the-art.

A limitation of our work is that there is no explicit modeling of the object functionality and human action in the current grasping field representation. In reality, a person holds an object differently based on different intentions. For instance, using a knife or passing it to someone else result in completely different human grasps. One promising future research direction is to incorporate human intention and object affordances into the grasping field for action specific grasps generation. Furthermore, 
we believe the proposed grasping field representation opens up avenues for several other future research directions. For instance, 3D human hand generation given only an object image and synthesizing the motion of hand-object interactions. 

% \newpage
\noindent \textbf{Acknowledgement.} We sincerely acknowledge Lars Mescheder and Michael Niemeyer for the detailed discussions on implicit function, Dimitrios Tzionas, Omid Taheri, and Yana Hasson for insightful discussions on hand interaction, Partha Ghosh and Qianli Ma for the help with VAE.
\textbf{Disclosure.} MJB has received research gift funds from Intel, Nvidia, Adobe, Facebook, and Amazon. While MJB is a part-time employee of Amazon, his research was performed solely at MPI. He is  an investor in Meshcapde GmbH.



% \section*{Broader impact}
% \label{sec:impact}

% Our method is a step towards tracking human hands and what they do in the world. This has many positive applications. For example, it could be used to analyze the performance of surgeons and give them guidance about better technique. It might one day provide an interface to a human-robot interaction system where the human guides the robot to learn new tasks. In these positive applications also lie the seeds of negative use cases. Training and improving performance can also turn into invasive monitoring of behavior. As these technologies evolve, the boundary between assisting and intruding will need to be defined.

% \section*{Acknowledgement}
% \label{sec:acknowledge}
% We sincerely acknowledge: Lars Mescheder and Michael Niemeyer for the detailed discussions on implicit function. Dimitrios Tzionas and Yana Hasson for insightful discussions on MANO and the baseline. Partha Ghosh and Qianli Ma for the implementation of VAE. Benjamin Pellkofer for IT/hardware supports.
